Adaptive Bounded Exploration and Intermediate Actions for Data Debiasing

The performance of algorithmic decision rules is largely dependent on the quality of training datasets available to them. Biases in these datasets can raise economic and ethical concerns due to the resulting algorithms' disparate treatment of different groups. In this paper, we propose algorithms for sequentially debiasing the training dataset through adaptive and bounded exploration in a classification problem with costly and censored feedback. Our proposed algorithms balance between the ultimate goal of mitigating the impacts of data biases -- which will in turn lead to more accurate and fairer decisions, and the exploration risks incurred to achieve this goal. Specifically, we propose adaptive bounds to limit the region of exploration, and leverage intermediate actions which provide noisy label information at a lower cost. We analytically show that such exploration can help debias data in certain distributions, investigate how {algorithmic fairness interventions} can work in conjunction with our proposed algorithms, and validate the performance of these algorithms through numerical experiments on synthetic and real-world data.

==> Proof_Thm1.tex <==
\begin{proof} \\
We detail the proof for label 0 estimates $\hat{\parameter}^0_t$, and discuss two cases while assuming (wlog) that the unknown $\parameter^y$ being estimated is the distribution's mean. First, if $\hat{\omega}^0_t$ is overestimated, i.e. $\hat{\omega}^0_t > \omega^0$. Note that we have $\theta_t \geq \hat{\omega}^0_t$. Then, as only agents with $x^\dagger\geq \theta_t$ are admitted, $\hat{\omega}^0_t$ may only be updated to stay the same or increase. Therefore, $\hat{\omega}^0_t$ will remain overestimated. 

Next consider the case that $\hat{\omega}^0_t$ is underestimated, $\hat{\omega}^0_t< \omega^0$. From $t$ on, consider the $T \gg t$ next steps. First, since each observation is independently drawn, we know that at time $t' = t,...,t+T$, 
$
x_{t'} - \mathbb E[X|X \geq \theta_{t'}]
$
forms a martingale; this is because of the independence of $x_{t'}$ and $\theta_{t'}$ when conditioned on the historical information, as well as the fact that $\mathbb E[x_{t'}] = \mathbb E[X|X \geq \theta_{t'}]$. 

By definition of $\omega^0$, we also know that 
$
\sum_{t'=t}^T \mathbb E[X|X \geq \theta_{t'}]  > T \cdot \omega^0
$. 
Denote the gap by $\Delta:=\frac{\sum_{t'=t}^T \mathbb E[X|X \geq \theta_{t'}]}{T} -   \omega^0$. Therefore using the Azuma-Hoeffding inequality we have 
\begin{align*}
    \mathbb P\Big(\sum_{t'=t}^T x_{t'} - \sum_{t'=t}^T \mathbb E[X|X \geq \theta_{t'}] \leq \delta \Big) \leq e^{\frac{-2\delta^2}{T-t+1}},
\end{align*}
for any $\delta < 0$. Letting $\delta = -\Delta \cdot (T-t+1)$, the above can be re-written as 
\begin{align*}
     \mathbb P&(\tfrac{1}{T-t+1} \sum_{t'=t}^T x_{t'} > \omega^0) >  1- e^{\left(-2\Delta^2(T-t+1)\right)} \underbrace{\rightarrow 1}_{T \rightarrow \infty}
\end{align*}
This proves that with high probability the mean of the new samples is higher than $\omega^0$. Therefore, at some time $T$ that is significantly higher than $t$, the new estimate $\hat{\omega}^0_T$ will be similar to $\frac{1}{T-t+1}\sum_{t'=t}^T x_{t'}$, which is higher than the true $\omega^0$. From our arguments for the overestimated case, from this point on, $\hat{\omega}^0_t$ will stay overestimated. The proof for $\hat{\omega}^1_t$ is similar. 
\end{proof}

==> discussion.tex <==
\section{More on Limitations, Extensions, and Social Impacts}\label{sec:extensions}

\paragraph{Limitations of Assumption~\ref{as:distributions}, and its extensions.} Our work, similar to the literature on multi-armed bandit learning, focuses on learning of a single unknown parameter (Assumption~\ref{as:distributions}). This assumption has also been adopted in prior work on studying biases in adaptively collected data~\citep{nie2018adaptively}. In addition, our problem is also similar to the commonly studied problem of estimating a \emph{location parameter} of a probability distribution in statistics. Despite the commonality, this assumption entails parametric knowledge of the underlying distribution with the other parameters such as variance or spread being known (or if unknown, immaterial) to the algorithm. This may be a limit in the applicability of our algorithm.  

As a first extension, in Appendix~\ref{app:two_parameters}, we have extended our algorithm and shown that it can debias the data in Gaussian distributions when both the mean and the variance of the distribution are unknown. Our algorithm still uses the same adaptive and bounded exploration mechanism outlined in Algorithm~\ref{def:db-alg}, and the LB set by Definition~\ref{def:UB-LB}. In particular, the bounds are still chosen so as to balance the estimated reference point (i.e. location parameter) of the distribution around its true parameter once correctly estimated; nonetheless, we show the data collected in this way can also be used to debias the variance. 

One potential drawback of this extension is that the debiasing of the variance is not \emph{robust}, in that although the algorithm debiases both parameters in the long-run, it initially {increases} the error in the variance estimate. This is because, initially, when observing samples outside of its believed range (due to a combination of incorrectly estimated means and variances), the algorithm increases its estimates of the variance to explain such samples. However, as the estimate of the mean is corrected, the variance can be reduced as well and become consistent with the collected observations. The extension of our bounded exploration and update procedure to account for both mean and variance debiasing and use of more robust estimators remain as an interesting direction of future work. 

Alternatively, the algorithm could use an input analyzer or distribution fit estimators of a given software to fit a desired distribution to the dataset available at the end of each round, by fixing the known parameters and fitting for the unknown parameters. Exploring this option, especially when additional parameters from the distribution are unknown, remains a direction of future research. 

\paragraph{One-dimensional features and threshold classifiers.} Our current analytical results have focused on one-dimensional feature data and threshold classifiers. Our experiments have also considered the use of our \texttt{active debiasing} algorithm on data with multi-dimensional features by performing a dimension reduction (e.g., as shown in the Adult dataset experiment). 

In general, such dimension reductions may lead to loss of information. To evaluate this in our setting, we run experiments on the Adult dataset with classifiers trained with and without performing dimension reduction. The experiments show only minimal loss in accuracy, with results as follows: 

$\bullet$ For the classifier trained through logistic regression without performing dimension reduction: the overall accuracy is 82.96\%, and the accuracy for advantaged (41762 samples) and disadvantaged (7080 samples) groups are 82.13\% and 88.26\%, respectively.

$\bullet$ For the classifier trained through logistic regression after performing dimension reduction: The overall accuracy is 78.07\%, and the accuracy for the advantaged and disadvantaged groups are 76.95\% and 84.69\%, respectively.

While this remains as a relative small ($\sim$ 5\%) loss in performance, better dimension reduction approaches, or debiasing algorithms that do not require feature dimension reduction, remain as interesting directions of future work. 

\paragraph{Extensions of our analytical results.} We conjecture that Theorem~\ref{thm:debiasing} on the performance of \texttt{active debiasing} can be extended to distributions beyond unimodal distributions. Further, the analytical study of weighted regret of our algorithm, and comparison against the regret incurred by our two baselines, which we have observed numerically in Section~\ref{sec:simulations}, remain as main directions of future work. 
As another future extension, we also propose considering a mixture of normal distributions with varying means and fixed covariances as the assumed form of the underlying distributions that are to be debiased. Such mixtures can be used to approximate other smooth probability density functions. An extension of our analytical results from unimodal distributions to these mixtures, together with extensions of our experimental results, could also address our algorithm's single unknown parameter limitation. 


\paragraph{Potential (negative) social impacts.} We have elaborated on the interplay of our algorithm with fairness constraints in Section~\ref{sec:two-group} as well as in our experiments. Accounting for the different impact of fairness constraints on the speed of debiasing of different groups may be a consideration when choosing to supplement debiasing efforts with fairness constraints, or vice versa. 

Also, a limitation of our algorithm for groups with smaller representation is discussed at the end of Section~\ref{sec:simulations}. In particular, we observed that in the \emph{Adult} dataset, as limited data is available on qualified, disadvantaged agents, the estimates on this population is not fully debiased despite the other estimates having been almost debiased. In other words, our debiasing algorithm is most effective on obtaining correct estimates on populations with sufficiently high representation. This may still be indirectly beneficial to the underrepresented populations, as by having better estimates on the represented population, the algorithm can better assess and impose fairness constraints. 


==> full_proof_active_debiasing.tex <==
\begin{proof}
We detail the proof for debiasing $\hat{f}_t^0$ (which happens using $x^\dagger \geq \text{LB}_t$ and $y^\dagger=0$); the proof for $\hat{f}_t^1$ is similar. 

\textbf{Part (a).} In time step $t+1$, with the arrival of a batch of $N_{t+1}$ samples in $[\text{LB}_t, \infty)$, the current estimate $\hat{\parameter}^0_t$ will be updated to $\hat{\parameter}^0_{t+1}$ based on the proportion of $\hat{\parameter}^0_t$ in the existing data. Denote the current left portion in $(\text{LB}_t, \hat{\parameter}^0_t)$ as $p_1 := \frac{\hat{F}^0(\hat{\parameter}^0_t) -\hat{F}^0(\text{LB}_t)}{\hat{F}^0(\theta_t)-\hat{F}^0(\text{LB}_t)}$. Based on Definition ~\ref{def:UB-LB}, we can also obtain the portion in $(\hat{\parameter}^0_t, \theta_t)$ denoted as $p_2 := \frac{\hat{F}^0(\theta_t) - \hat{F}^0(\hat{\parameter}^0_t)}{\hat{F}^0(\theta_t)-\hat{F}^0(\text{LB}_t)} = p_1$. We consider the following cases:

\underline{Case 1 (Perfectly estimated)}: $\hat{\parameter}_t^0=\parameter^{0}$. When the estimates are perfectly estimated, we will have both $\theta_t$ and $\text{LB}_t$ perfectly estimated too. Hence, we have $F^0(\theta_t) - F^0(\hat{\parameter}_t^0) = F^0(\hat{\parameter}_t^0) - F^0(\text{LB}_t)$ such that $p_1 = p_2$. Thus, $\mathbb{E}[\hat{\parameter}^0_{t+1}]=\parameter^0$. 
Hence, once the parameter is correctly estimated,  $\hat{f}_t^0$ is not expected to shift from $f^0$. 

\underline{Case 2 (Underestimated)}: $\hat{\parameter}_t^0<\parameter^{0}$. Under the unimodel distribution and single parameter assumption, since the arriving batch of data comes from the true distribution, $F^0(\text{LB}_t), F^0(\hat{\parameter}_t^0), F^0(\theta_t)$ will be smaller than $\hat{F}^0(\text{LB}_t), \hat{F}^0(\hat{\parameter}_t^0), \hat{F}^0(\theta_t)$, respectively. Moreover, since we have $\text{LB}_t \leq \hat{\parameter}_t^0 \leq \theta_t \leq \hat{\parameter}^1_t$, {then $F^0(\theta_t) - F^0(\hat{\parameter}_t^0) \geq F^0(\hat{\parameter}_t^0) - F^0(\text{LB}_t)$ such that $p_2 \geq p_1$. Hence, more samples are expected to be observed in range of $(\hat{\parameter}^0_t, \theta_t)$ so that the $\hat{\parameter}^0_t$ is expected to shift up.  Hence, we have $\mathbb{E}[\hat{\parameter}^0_{t+1}] \geq \hat{\parameter}^0_{t}$.} 

\underline{Case 3 (Overestimated)}: $\parameter^{0} <  \hat{\parameter}_t^0$.  Through similar analysis as \underline{Case 2 (Underestimated)}, we can obtain $\mathbb{E}[\hat{\parameter}^0_{t+1}] \leq \hat{\parameter}^0_{t}$.

\textbf{Part (b).} We first show that the converging sequence converges to the true estimates. 

By the construction of the bounds in Definition ~\ref{def:UB-LB}, the estimated parameter $\hat{\parameter}^0_{t}$ is the $\alpha$-th percentile of $\hat{f}_t^0$, the median in the interval $[\text{LB}_t, \theta_t]$ and  some percentile in the interval $[\text{LB}_t, \infty)$; we therefore first find their distribution accordingly. Assume there are $N_t=m+n+1$ points in the interval $[\text{LB}_t, \infty)$ with $m$ and $n$ samples below and above $\hat{\parameter}^0_{t}$ respectively. More specifically, for these $n$ samples, there are $m$ samples between $[\hat{\parameter}^0_{t}, \theta_t]$ and $n-m$ samples above $\theta_t$. Based on the probability distribution of order statistics in $[\text{LB}_t, \theta_t]$, denote three possibilities $X$, $Y$, $Z$ denoting the number of samples below, on, and above the $\hat{\parameter}^0_{t}$, respectively, having probabilities $p= \tfrac{F^0(\hat{\parameter}^0_{t})-F^0(\text{LB}_t)}{F^0(\theta_t)-F^0(\text{LB}_t)}$, $q=\tfrac{f^0(\hat{\parameter}^0_{t})}{F^0(\theta_t)-F^0(\text{LB}_t)}$, and $r=\tfrac{F^0(\theta_t)-F^0(\hat{\parameter}^0_{t})}{F^0(\theta_t)-F^0(\text{LB}_t)}$.  Since the distributions are continuous, the probability of multiple samples being exactly on $\hat{\parameter}^0_{t}$ is zero. Therefore, the pdf of $\hat{\parameter}^0_{t}$ can be found based on the density function of the trinomial distribution: 
{\begin{align}
\mathbb P(\hat{\parameter}^0_{t}=\nu) \mathrm{d}\nu= \frac{(2m+1)!}{m!m!}(\tfrac{F^0(\nu)-F^0(\text{LB}_t)}{F^0(\theta_t)-F^0(\text{LB}_t)})^m(\tfrac{F^0(\theta_t)-F^0(\nu)}{F^0(\theta_t)-F^0(\text{LB}_t)})^m \tfrac{f^0(\nu)}{F^0(\theta_t)-F^0(\text{LB}_t)}\mathrm{d}\nu
\label{eq:median-pdf-trinomial}
\end{align}}
From the above, we can see that the density function of the $\hat{\parameter}^0_{t}$ is a beta distribution with $\alpha=m+1, \beta=m+1$, pushed forward by $H(\nu):=\tfrac{F^0(\nu)-F^0(\text{LB}_t)}{F^0(\theta_t)-F^0(\text{LB}_t)}$; this is the CDF of the truncated $F^0$ distribution in $[\text{LB}_t, \theta_t]$. In other words, using $G$ to denote the Beta distribution's CDF, $\hat{\parameter}^0_{t}$ has CDF $G(H(\nu))$, and by the chain rule, pdf $g(H(\nu))h(\nu)$.  

It is known ~\cite{maritz1978note} that for samples located in the range of $[\text{LB}_t, \theta_t]$, the sampling distribution of the median becomes asymptotically normal with mean $(\parameter^0)'$ and variance $\frac{1}{4(2m+3)H((\parameter^0)')}$, where $(\parameter^0)'$ is the median, the truncated $F^0$ distribution in $[\text{LB}_t, \theta_t]$. If the sequence of $\{\hat{\parameter}^0_t\}$ produced by our \texttt{active debiasing} algorithm converges, by Definition ~\ref{def:UB-LB}, the thresholds $\text{LB}_t$ and $\theta_t$ will converge as well; As $t\rightarrow \infty$, $\epsilon_t \rightarrow 0$, $2m+1\rightarrow\infty$ in this interval, the variance becomes zero, and  $\hat{\parameter}^0_{t+1}\rightarrow (\parameter^0)'$. By Definition ~\ref{def:UB-LB}, it must be that the median $(\parameter^0)'$ of $H$ is equal to $\parameter^0$. Therefore, $\hat{\parameter}^0_{t+1}\rightarrow \parameter^0$.

Lastly, we show that the sequence of estimates $\{\hat{\parameter}^0_t\}$ is a converging sequence. Consider the sequence of estimates $\{\hat{\parameter}^0_t\}$, and separate into the two disjoint subsequences $\{\hat{y}^0_t\}$ denoting the parameters that are underestimated with respect to the true $\parameter^0$, and $\{\hat{z}^0_t\}$ denoting those that are overestimated.

We now show that the sequence of underestimation errors, $\{\Delta^y_t\} : = \{\parameter^0- \hat{y}^0_t\}$ and the sequence of overestimation errors, $\{\Delta^z_t\} : = \{\hat{z}^0_t-\parameter^0\}$, are supermartingales. We detail this for $\{\Delta^y_t\}$. Consider two cases: 
\begin{itemize}
    \item First, assume the update $\hat{y}^0_{t+1}$ is the next immediate update after $\hat{y}^0_{t}$ in the original sequence $\{\hat{\parameter}^0_t\}$; that is, an underestimated $\hat{y}^0_{t}$ has been updated to a parameter that continues to be an underestimate. In this case, by Part (a), $\mathbb{E}[\hat{y}^0_{t+1}|\hat{y}^0_{t}]\geq \hat{y}_t^0$, and therefore, $\mathbb{E}[\Delta^y_{t+1}|\Delta^y_{t}]\leq \Delta^y_t$. 
    \item Alternatively assume $\hat{y}^0_{t+1}$ is not obtained immediately from $\hat{y}^0_{t}$; that is, $\hat{y}^0_{t+1}$ has been obtained as a result of an update from an overestimated parameter. We note that now, $\hat{y}^0_{t+1}\geq \hat{y}_t^0$. This is because either no new estimates have been obtained between $\hat{y}_t^0$ and the true parameter $\parameter^0$ since the last time the parameter was underestimated, in which case, it must be that $\hat{y}^0_{t+1}=\hat{y}_t^0$. Otherwise, a new estimate in $[\hat{y}_t^0, \parameter^0]$ has been obtained, in which case, again, $\mathbb{E}[\hat{y}^0_{t+1}|\hat{y}^0_{t}]\geq \hat{y}_t^0$. In either case, $\mathbb{E}[\Delta^y_{t+1}|\Delta^y_{t}]\leq \Delta^y_t$. 
\end{itemize}

Therefore, by the Doobs Convergence theorem, the supermatingales $\{\Delta^y_t\}$ and $\{\Delta^z_t\}$ converge to random variables $\Delta^y$ and $\Delta^z$. By the same argument as the beginning of the proof of this part, these are asymptotically normal with mean zero and with variances decreasing in the number of observed samples in their respective intervals. Therefore, $\Delta^y\rightarrow 0$ and $\Delta^z\rightarrow 0$ as $N\rightarrow \infty$, and therefore $\{\hat{\parameter}^0_t\}$ converges to $\parameter$. 
\end{proof}

==> related-additional.tex <==
\section{Additional and Detailed Related Work}\label{app:related-additional}

\textbf{Interplay of fairness criteria and data biases.} Our analysis in Section~\ref{sec:two-group}, similar to those of \citet{blum2020recovering} and \citet{jiang2020identifying}, also considers the interplay between algorithmic fairness rules and data biases. \citet{blum2020recovering} show that certain fairness constraints can \emph{themselves} be interpreted as enabling debaising of the underlying estimates. Also, both works 
study data bias arising due to the \emph{labeling} process and propose reweighting techniques to address it. Our work differs from these from two main aspects. First, we model biases as changes in feature-label distributions, in contrast to the assumption of noisy labels in these works. Second, we introduce a statistical debiasing technique based primarily on exploration, which is orthogonal to the social debiasing achieved through fairness constraints. Our proposed model and algorithm therefore complement these works. 

\textbf{Long-term fairness and bias in algorithmic decision making:} The majority of works on fair algorithmic decision making have focused on achieving fairness in a one-shot setting (i.e. without regards to the long-term effects of the proposed algorithms); see e.g.~\citep{hardt2016equality,dwork2012fairness,corbett2017algorithmic}. Some recent works have studied long-term impacts of fairness on disparities, group representation, and strategic manipulation of features, as a result of adopting fairness measures~\citep{liu2018delayed,zhang2019group,liu2020disparate}. Our work contributes to this line of research, by analyzing the long-term effects of imposing fairness constraints on data collection and debiasing efforts. 

\textbf{Biases in adaptively collected data:} A few other works have, similar to our work, explored the question of biases induced by a decision rule on data collection. \citet{deshpande2018accurate} study inference in a linear model with adaptively collected data; in contrast to our proposed method, their work focuses on debiasing of an estimator, rather than modifying the decision rule used to collect the data.  \citet{nie2018adaptively} study the problem of estimating statistical parameters from adaptively collected data. Their proposed adaptive data collection method, which also similar to ours (Assumption~\ref{as:distributions}) is used for single-parameter estimation, is one of online debiasing; our proposed data collection methods however differ. In particular, our focus is on accounting for multiple subgroups as well as fairness considerations. More importantly, we propose a \emph{bounded} exploration strategy, which accounts for the risks of exploration decisions and limits the depth of exploration; this method of exploration is different from the random exploration used to collect the data in~\citep{nie2018adaptively}, to which their proposed debiasing algorithms based on data splitting and modified maximum likelihood estimators are applied.  

\textbf{Active learning}: Our work is also related to the active learning literature. \citet{balcan2007margin} study the sample complexity of labeled data required for active learning, \citet{kazerouni2020active} propose an algorithm involving exploration and exploitation-based adaptive sampling, verifying it using simulations, \citet{abernethy2022active} propose an active sampling and re-weighting technique by sampling from the worst off group at each step with the goal of building a computationally efficient algorithm with strong convergence guarantees to improve the performance on the disadvantage (highest loss) group while satisfying the notion of min-max fairness, \citet{noriega2019active} propose an adaptive fairness approach, which adaptively acquires additional information according to the needs of different groups or individuals given information budgets, to achieve fair classification. Similar to the approaches of these papers, we also compensate for adaptive sampling bias through exploration (by admitting individuals who would otherwise be rejected). Comparing to all these literature, we start with a biased dataset, and we primarily focus on recovering the true distribution by bounded exploration, accounting for the cost of exploration, avoiding the adaptive sampling bias, and consider fairness issues as orthogonal to our data collection procedure (and as such, can apply our procedure to debiasing the estimates on a single group). 

\textbf{Selective labeling bias}: \citet{lakkaraju2017selective} address the problem of evaluating the performance of predictive model under the selective labeling problem. They propose a contraction technique to compare the performance of the predictive model and human judge while they are forced to have the same acceptance rate. \citet{de2018learning} study the problems arising due to selective labeling. Similar to us, they propose a data augmentation scheme by adding more samples that would be more likely rejected (we refer to this as exploration) to correct the sample selection bias. Their proposed data augmentation technique is similar to our bounded exploration, but it differs in its selection of samples in that it adds samples that would be more likely to be rejected. 

\textbf{Fair learning}: \citet{kallus2018residual} show that residual unfairness remains even after the adjustment for fairness when policies are learned from a biased dataset. They propose a re-weighting technique (similarly, re-weighing ideas are explored in \citep{blum2020recovering} and \citep{jiang2020identifying}) to solve the residual unfairness issue while accounting for the censoring/adaptive sampling bias. 

\textbf{Online mean estimation:} Compared to this literature, the main technical challenges of our proposed bounded exploration in online mean estimation is that it involves evaluating the behavior of statistical estimates based on data collected from a truncated distribution with \emph{time-varying} truncation. More specifically, our data collection interval is bounded and truncated (which has been considered in some prior work on distribution/mean estimation as well, e.g., \citet{lai1991estimating}) but our exploration interval $[LB_t, \infty)$ is itself adaptive (which we believe is the main new aspect) and is what has motivated our analysis in a finite sample regime in Theorem 3. Our focus on the interplay of fairness constraints with online estimation efforts (Proposition 1) is also new compared to this existing literature.

\textbf{Performative prediction:} Finally, the recent line of work on performative prediction proposed by \citet{perdomo2020performative}  also considers the effects of algorithmic decisions on the underlying population's features-label distributions. In particular, the choice of the ML model can cause a shift in the data distribution, and the goal of this work is to identify the stable ML model parameter that is attained at a fixed point of the algorithm-population interactions. In contrast, our focus is on \emph{pre-existing} and unchanging distribution shifts in the data, which our \texttt{active debiasing} algorithm aims to correct over time. Therefore, our algorithm could be considered as a debiasing method to be used when such performative shifts are present in the data, but are unaccounted for: If distribution shifts happen relatively slower than our debiasing algorithm's convergence speed, our \texttt{active debiasing} could be used to recover correct estimates of the underlying distribution, the estimates of which might be biased due to performative distribution shifts. 


